L3GS: Layered 3D Gaussian Splats for Efficient 3D Scene Delivery

Traditional 3D content representations include dense point clouds that consume large amounts of data and hence network bandwidth, while newer representations such as neural radiance fields suffer from poor frame rates due to their non-standard volumetric rendering pipeline. 3D Gaussian splats (3DGS) can be seen as a generalization of point clouds that meet the best of both worlds, with high visual quality and efficient rendering for real-time frame rates. However, delivering 3DGS scenes from a hosting server to client devices is still challenging due to high network data consumption (e.g., 1.5 GB for a single scene). The goal of this work is to create an efficient 3D content delivery framework that allows users to view high quality 3D scenes with 3DGS as the underlying data representation. The main contributions of the paper are: (1) Creating new layered 3DGS scenes for efficient delivery, (2) Scheduling algorithms to choose what splats to download at what time, and (3) Trace-driven experiments from users wearing virtual reality headsets to evaluate the visual quality and latency. Our system for Layered 3D Gaussian Splats delivery L3GS demonstrates high visual quality, achieving 16.9% higher average SSIM compared to baselines, and also works with other compressed 3DGS representations.

==> shepherd_response_xuechen.tex <==
We thank the reviewers for the constructive comments. Below, we outline the plan of addressing each suggested improvement for the camera-ready version of our paper.

Main change:

We will add more detailed clarification about bandwidth prediction, utility function design(RA, W2), and how user behavior influences the SSIM(RA, W4) 

We will also add a future work and limitation section discussing how to extend the framework to multi-user scenarios, unpredictable user behavior challenges and potential methods of more accurate viewport/bandwidth prediction (RA, W1). 


Response to main comments

(1) Clarify and evaluate bandwidth prediction.
We appreciate the reviewers' comments on clarifying the bandwidth prediction component of our framework. For the camera-ready version, we will provide a more comprehensive explanation of our bandwidth prediction model in Section 3.4. Specifically, we will:
1. Add explanation and analysis to elaborate more on the harmonic mean approach used for bandwidth prediction and its integration with the scheduler. We will also discuss the limitation and advantage of our bandwidth prediction method.

2. We will provide additional experimental results to demonstrate the system’s robustness under fluctuating network conditions. Specifically, we will include three additional figures:
	•	Fig. 1: Visual quality (SSIM) across bandwidth traces with three levels of variance—low, medium, and high.
    •	Fig. 2: Bandwidth prediction accuracy (absolute error) across bandwidth traces with three levels of variance—low, medium, and high.
    •	Fig. 3: Relationship between visual quality (SSIM) and bandwidth prediction accuracy (absolute error) across different bandwidth traces.

3. We will add a section titled “Limitations and Future Work” where we will discuss the potential of the framework in real-world network environments. Specifically, we will consider varying network conditions, such as packet loss, handovers, and other fluctuations rather than only relying on trace-based predictions. 
% Xuechen's main change: merge original 2 and 3. Add new 3 discussing actual network
% 1. Elaborate more on the harmonic mean approach used for bandwidth prediction and its integration with the scheduler. 
% 2. Provide more evaluation results to show the system's robustness under fluctuating network conditions. Specificlly, we will provide measurement results of the bandwidth traces' variance's influence on the visual quality (SSIM) and the accuracy (absolute error) of the bandwidth prediction to demonstrate the system's robustness.
% 3. Provide more evaluation results to show the system's robustness under inaccurate estimations. Specifically, we will provide system performance evaluation under different bandwidth prediction accuracy.

(2) Address viewport prediction concerns.
We acknowledge the concerns regarding the accuracy of viewport prediction. 
To address these, we will:
1. We will expand our discussion on why we chose a linear regression-based viewport prediction model. In short, we require a predictor with low latency that can easily adapt to different traces without needing a large number of training samples. Therefore, advanced machine learning models are not suitable for our use case. 
2. We appreciate the suggestions about mitigation strategies such as incorporating the AR/VR context. However, as mentioned, these advanced strategies come with their own limitations. We will discuss these in our newly added “Limitations and Future Work” section.
3. We will also highlight the ablation results in Figure 17, demonstrating that our linear regression-based viewport prediction achieves visual quality (SSIM) comparable to that of using the ground-truth viewport, even including erratic user movement traces. This directly addresses concerns regarding the performance of the viewport prediction model.
% Xuechen's main change: I don't agree with the mitigation strategies suggestions. So what I write is different from the original version. we have some discussion in google drive comments


% 1. Expand our discussion in Section 3.3 to discuss the limitations of linear regression-based viewport prediction, particularly in scenarios with erratic user movement. //xuechen comment: limitations and strength? highlight latency and sample size issue. We can't use large ml models.
% 2. Discuss possible mitigation strategies such as hybrid models combining linear regression with machine learning techniques for longer-term predictions. These mitigations will be discussed as future improvements.  //xuechen comment: combining linear regression with machine learning techniques sounds weird to me. 
% // 3. Include new evaluation results comparing the system’s performance under perfect viewport prediction to show the system's robustness.
% // efficient/light-weight
% // remove 3

% // add a future improvements/limitation section?

(3) Include comparison with existing work.
Thank you for your suggestion. 
To strengthen this comparison, we will provide a more detailed analysis of how our work relates to and differs from existing approaches.
% We recognize the importance of comparing our work with other existing work. 
% 1. Provide a detailed comparison between our layered 3D Gaussian splat framework and other existing scalable techniques.

% // add a discussion section?

Individual responses
Most of the concerns have been addressed in the main response. Here, we will only respond to specific concerns.
Reviewer A
1. We will add detailed explanation and ablation study of the utility function design. 
2. We appreciate the suggestion to evaluate the system from the perspective of user perception. We will include these insights in our new section, “Limitations and Future Work.”
Reviewer B
All concerns have been addressed in the main response.
Reviewer C
1. We acknowledge the concern about the dependency on precomputed utilities. We will clarify that we cluster and precompute all possible viewports, ensuring there are no unexpected user viewports. However, we also recognize the limitations of relying on precomputed utilities, which we will discuss in our new section, “Limitations and Future Work.”
2. Thank you for the suggestion regarding scalability in multi-user environments. We will include a discussion of this in our new section, “Limitations and Future Work.”
Reviewer C
All concerns have been addressed in the main response.
% Reviewer A
% Weakness (4)
% 1.
% We acknowledge that the linear regression-based viewport prediction within a short history window is a simple approach. 
% The primary motivation for using this approach was to realize efficient real-time prediction in AR/VR environments. Linear regression-based viewport prediction is lightweight and computationally efficient, which makes it suitable for mobile depolyment. Due to the resource constraints of the mobile environment, more complex viewport prediction methods are usually not suitable for mobile deployment due to their as they usually need more computational resource and will introduce longer latency.
% However, we do recognize the potential benefits of incorporating AR/VR-specific contexts. We will clarify our design rationale and discuss how AR/VR-specific contexts (e.g. user preferences) could enhance prediction accuracy. 

% // in the demo, the viewport prediction is actually done on the server side, will this cause problem?
% // add a future improvements/limitation section?

% 2.
% Multiplication reflects the compounded nature of these attributes: a splat that is close, highly visible in the viewport, and has high opacity is far more critical than one that scores highly on only one or two factors. An additive or weighted sum approach would fail to capture these compounded effects, overemphasizing individual factors. 
% Regarding the use of global significance scores, they are viewport-independent and primarily useful for general importance ranking. Our utility function is designed to be dynamic and viewport-specific, adapting to real-time user movements. Besides, we already included opacity as part of the utility function design, which is also an important component of the global significance scores.
% To address this feedback, we will add discussions to justify the current utility design and discuss possible further improvements.

% // we experiment both xxx
% // how to justify not using global significace scores
% // Is opacity part of the global significance scores?

% 3. 
% We appreciate the suggestion to evaluate the system from the perspective of user perception. While our current evaluation relies on SSIM for performance evaluation, we acknowledge its limitationsin capturing subjective user experiences. 
% User studies would provide valuable insights into how significant the perceived improvements are in real-world scenarios. For the camera-ready version, we will include a discussion proposing a user study design as future work. 

% // add a future improvements/limitation section?

% 4.
% We agree that robustness to erratic user behaviors is a critical aspect of 3D scene delivery. 
% Our layered design prioritizes critical splats in the predicted viewport, potentially making it more adaptive to challenging behaviors than models requiring complete downloads. For the camera-ready version, we will discuss possible future improvements to improve the system's robustness to erratic user behaviors.
% As mentioned in the response to the main comments, we will also analyze how viewport prediction accuracy affects robustness and suggest ways to further improve adaptability

% // As mentioned in the response to main comments... Is the wording ok? Or I need to repeat everything?
% // we will not add quantitative results right?
% // which model?
% // not really address the concern...
% // leave for future work

% Reviewer B
% Weakness (2)
% 1.
% We appreciate the suggestion to provide more details on how the framework performs under varying network conditions. As mentioned in the main comments, we will provide more evaluation results to show the system's robustness under fluctuating network conditions. Specificlly, we will provide measurement results of the bandwidth traces' variance's influence on the visual quality (SSIM) and the accuracy (absolute error) of the bandwidth prediction to demonstrate the system's robustness.

% // what about the packet loss etc. pointed out in the comments?
% // bw already consider pkt loss from the application level
% // As mentioned in the main comments... Copied from the main comments/rewrite?

% 2.
% We agree that the current ablation study could be more comprehensive, particularly in testing adaptability under varying conditions such as scene complexity.
% We will discuss this as parts of the limitations of our paper and discuss possible future improvements of improving the system's adaptability under varying conditions like scene complexity.

% // not running more experiment
% // not directly address the problem

% Reviewer C
% Weakness (4)
% 1.
% We recognize that the viewport prediction based on linear regression may struggle with complex user movements, potentially leading to suboptimal scheduling decisions. We choose linear regression for viewport prediction is due to its light weight nature and low computational requirements, which can easily fit the mobile enviroment's resource constraints. In the camera-ready version, we will discuss the rationales and the limitations of using linear regression as well as possible future improvements (e.g. using machine learning for prediction) for enhancing the prediction accuracy.
% // same as (2)

% 2.
% We agree that the current bandwidth predictor might not capture sudden fluctuations accurately, potentially impacting scheduling efficiency in highly variable network conditions. In the camera-ready version, we will provide more evaluation results to show the system's robustness under fluctuating network conditions. Specificlly, we will provide measurement results of the bandwidth traces' variance's influence on the visual quality (SSIM) and the accuracy (absolute error) of the bandwidth prediction to demonstrate the system's robustness.
% Additionally, We will provide more evaluation results to show the system's robustness under inaccurate estimations. Specifically, we will conduct ablation study to compare the system performance under perfect network bandwidth prediction and provide the corresponding results. Possible limitations and future improvements of the current bandwidth predictor will also be discussed.

% // same as (1), copied
% // do we really capture the fluctuations? With interpolation (I assume linear), there seems no fluctuation.

% 3.
% Precomputing utilities for splats provides a practical solution for real-time scheduling, but it limits adaptability to unexpected user behaviors or dynamic scene complexity. Depending on the scene size and complexity, real-time computation may have better performance than the precomputation or vice versa. In the camera-ready version, we will discuss the trade-offs between precomputed and real-time utility calculations. We will also discuss possible future improvements (e.g. using a hybrid approach).

% 4.
% We agree that the scalability to multi-user environments remains unexplored. In the camera-ready version, we will discuss the challenges and potential solutions for adapting the framework to multi-user scenarios, such as shared splat prioritization or user-specific scheduling. We will also discuss how existing features in the current framework (e.g. segmentation) could be leveraged to optimize performance in multi-user scenarios.


% Reviewer D
% Weakness (2)
% 1.
% We appreciate your observation about recent work on layered Gaussian splats. While our work shares similarities with these methods, our contributions are distinct in several ways:
% Our approach uniquely integrates object-level segmentation, enabling the scheduler to prioritize splats based on semantic importance, rather than solely relying on global utility scores.
% Our scheduler takes both viewport and bandwidth into consideration when doing the progressive scene delivery instead of simply deliver the layer one by one based on the bandwidth availability. 

% // two points kind of share some overlaps
% In the camera-ready version, we will a detailed comparison with the referenced work and other recent approaches to layered Gaussian splats.
% // add in which section?

% 2.
% (1) Clarify and evaluate bandwidth prediction.
% We appreciate the reviewers' comments on clarifying the bandwidth prediction component of our framework. For the camera-ready version, we will provide a more comprehensive explanation of our bandwidth prediction model in Section 3.4. Specifically, we will:
% 1. Elaborate more on the harmonic mean approach used for bandwidth prediction and its integration with the scheduler.
% 2. Provide more evaluation results to show the system's robustness under fluctuating network conditions. Specificlly, we will provide measurement results of the bandwidth traces' variance's influence on the visual quality (SSIM) and the accuracy (absolute error) of the bandwidth prediction to demonstrate the system's robustness.
% 3. Provide more evaluation results to show the system's robustness under inaccurate estimations. Specifically, we will conduct ablation study to compare the system performance under perfect network bandwidth prediction and provide the corresponding results.

% (2) Address viewport prediction concerns.
% We acknowledge the reviewers’ concerns regarding viewport prediction accuracy. 
% To address these, we will:
% 1. Expand our discussion in Section 3.3 to discuss the limitations of linear regression-based viewport prediction, particularly in scenarios with erratic user movement.
% 2. Discuss possible mitigation strategies such as hybrid models combining linear regression with machine learning techniques for longer-term predictions. These mitigations will be discussed as future improvements. 
% 3. Include new evaluation results comparing the system’s performance under perfect viewport prediction to show the system's robustness.

% // same as (1) and (2), do we need to modify it a bit.

% 3.
% We appreciate the suggestion to explore alternative scalable approaches, such as MDC (Multiple Description Coding), where layers collaboratively increase quality without strict ordering. While this is outside the scope of the current work, we agree that such approaches may offer advantages in lossy networks or multi-user settings. In the camera-ready version, we will include this as possible future improvements.

% // are we going to send the comments separately? (e.g. add thanks xxx for reviewers.)

==> system_design_backup.tex <==
\section{System Design}

Overview - Angela

\subsection{Layered 3D Gaussians models}
To create a 3D scene with different level-of-details (LOD) models, we first tried to understand the significance of 3D Gaussians features to visual quality. We categorize the features into view-independent and view-dependent ones and also examine the matrix trade-offs of distance and opacity.
\begin{itemize}
    \item View-independent: 3D Gaussians size, opacity, RGB sum, size*opacity
    \item View-dependent: distance, orientation difference, pixel size
    \item Distance-opacity matrix trade-offs: closer/further and transparent/opaque
\end{itemize}
Given a trained 3D Gaussians scene, we sort the total splats (1.1 million) by different combinations of features, render the top [10, 20, ..., 100]\% features of the splats, and compute the SSIM. In~\autoref{fig:sorted-splats}, we show a trend of more splats contributing to higher visual quality, and opacity, and size\_opacity can increase the visual quality more quickly than other variables. 

However, we also compared the same scene with different numbers of total splats from different densification thresholds set when training the 3D Gaussians from scratch (top magenta line, from 70K up to 2.7M). The result indicates that a trained scene with fewer splats can reach higher visual quality than the top k\% of splats.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{No segmentation. Seperate: Each level of the models is trained separately, with no weight sharing. sort:
Loaded the official pretrained model, sorting all the splats with the v\_important score. layered: Progressive training. Each level of the models are trained with weight sharing.}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|lll|lll|lll|}
\hline
\multirow{2}{*}{}        & \multirow{2}{*}{\# of splats} & \multicolumn{3}{l|}{psnr} & \multicolumn{3}{l|}{ssim} & \multicolumn{3}{l|}{lpips} \\ \cline{3-11} 
                  &                               & \multicolumn{1}{l|}{separate} & \multicolumn{1}{l|}{sort} & layered & \multicolumn{1}{l|}{separate} & \multicolumn{1}{l|}{sort} & layered      & \multicolumn{1}{l|}{separate} & \multicolumn{1}{l|}{sort} & layered       \\ \hline
\multirow{4}{*}{Bicycle} & 45000        &\multicolumn{1}{l|}{21.3155} & \multicolumn{1}{l|}{14.1800/15.3934} &  21.3155 & \multicolumn{1}{l|}{0.464} & \multicolumn{1}{l|}{0.3136/0.3639} &  0.4647  &\multicolumn{1}{l|}{0.5710} & \multicolumn{1}{l|}{0.6124/0.5986} &   0.5710  \\ \cline{2-11} 
                         & 90000        &\multicolumn{1}{l|}{21.7718} & \multicolumn{1}{l|}{14.6635/20.9761} &  21.8171 &  \multicolumn{1}{l|}{0.4902} & \multicolumn{1}{l|}{0.3425/0.4037} & 0.4939  &\multicolumn{1}{l|}{0.5310} & \multicolumn{1}{l|}{0.5721/0.5424} & 0.5238 \\ \cline{2-11} 
                         & 135000       &\multicolumn{1}{l|}{22.0827} & \multicolumn{1}{l|}{15.0201/21.8416} & 21.9498  &  \multicolumn{1}{l|}{0.5101} & \multicolumn{1}{l|}{0.3634/0.4896} & 0.4979 &\multicolumn{1}{l|}{0.4997} & \multicolumn{1}{l|}{0.5455/0.5001} & 0.5026\\ \cline{2-11} 
                         & 180000       &\multicolumn{1}{l|}{22.3010} & \multicolumn{1}{l|}{15.3178/22.3010} & 22.0283& \multicolumn{1}{l|}{0.5272} & \multicolumn{1}{l|}{0.3796/0.5272} & 0.5168   &\multicolumn{1}{l|}{0.4743} & \multicolumn{1}{l|}{0.5252/0.4743} &  0.4903 \\ \hline
\multirow{4}{*}{Bonsai} & 45000        &\multicolumn{1}{l|}{25.9307} & \multicolumn{1}{l|}{18.1935} &  25.9307 & \multicolumn{1}{l|}{0.7978} & \multicolumn{1}{l|}{0.6392} &   0.7978 &\multicolumn{1}{l|}{0.3717} & \multicolumn{1}{l|}{0.4585} & 0.3717    \\ \cline{2-11} 
                         & 90000        &\multicolumn{1}{l|}{27.9939} & \multicolumn{1}{l|}{20.2791} & 27.6851  & \multicolumn{1}{l|}{0.8564} & \multicolumn{1}{l|}{0.7070} &  0.8536 & \multicolumn{1}{l|}{0.3069} & \multicolumn{1}{l|}{0.3997} & 0.3156 \\ \cline{2-11} 
                         & 135000       &\multicolumn{1}{l|}{29.1594} & \multicolumn{1}{l|}{21.8486} & 28.3041  &  \multicolumn{1}{l|}{0.8874} & \multicolumn{1}{l|}{0.7589} & 0.8757  &\multicolumn{1}{l|}{0.2692} & \multicolumn{1}{l|}{0.3579} & 0.2875 \\ \cline{2-11} 
                         & 180000       &\multicolumn{1}{l|}{30.0454} & \multicolumn{1}{l|}{23.1811} & 28.6004& \multicolumn{1}{l|}{0.9065} & \multicolumn{1}{l|}{0.7992} &   0.8852 &\multicolumn{1}{l|}{0.2446} & \multicolumn{1}{l|}{0.3240} & 0.2731  \\ \hline
\multirow{4}{*}{Counter} & 45000        &\multicolumn{1}{l|}{24.8746} & \multicolumn{1}{l|}{18.2148} & 24.8746  & \multicolumn{1}{l|}{0.7892} & \multicolumn{1}{l|}{0.6439} &    0.7892 &\multicolumn{1}{l|}{0.3767} & \multicolumn{1}{l|}{0.4468} &    0.3767 \\ \cline{2-11} 
                         & 90000        &\multicolumn{1}{l|}{26.4120} & \multicolumn{1}{l|}{20.4224} & 26.4103  & \multicolumn{1}{l|}{0.8310} & \multicolumn{1}{l|}{0.7060} &  0.8345 &\multicolumn{1}{l|}{0.3197} & \multicolumn{1}{l|}{0.3881} & 0.3155 \\ \cline{2-11} 
                         & 135000       &\multicolumn{1}{l|}{27.2702} & \multicolumn{1}{l|}{21.9577} & 26.8476  & \multicolumn{1}{l|}{0.8549} & \multicolumn{1}{l|}{0.7480} & 0.8508  &\multicolumn{1}{l|}{0.2863} & \multicolumn{1}{l|}{0.3497} & 0.2914 \\ \cline{2-11} 
                         & 180000       &\multicolumn{1}{l|}{27.7992} & \multicolumn{1}{l|}{23.1797} & 27.0763 & \multicolumn{1}{l|}{0.8708} & \multicolumn{1}{l|}{0.7810} &  0.8600  &\multicolumn{1}{l|}{0.2634} & \multicolumn{1}{l|}{0.3196} & 0.2764  \\ \hline
\multirow{4}{*}{Train} & 45000        &\multicolumn{1}{l|}{19.6034} & \multicolumn{1}{l|}{14.6942/15.8078} & 19.6034  &  \multicolumn{1}{l|}{0.6389} & \multicolumn{1}{l|}{0.4901/0.5360} &    0.6389 &\multicolumn{1}{l|}{0.4279} & \multicolumn{1}{l|}{0.5081/0.4750} &  0.4279   \\ \cline{2-11} 
                         & 90000        &\multicolumn{1}{l|}{20.7128} & \multicolumn{1}{l|}{16.2860/19.0613} & 20.6103  &\multicolumn{1}{l|}{0.7049} & \multicolumn{1}{l|}{0.5612/0.6606} & 0.7002  &\multicolumn{1}{l|}{0.3588} & \multicolumn{1}{l|}{0.4396/0.3800} & 0.3645 \\ \cline{2-11} 
                         & 135000       &\multicolumn{1}{l|}{21.2883} & \multicolumn{1}{l|}{17.3991/21.0321} & 20.9375  &\multicolumn{1}{l|}{0.7404} & \multicolumn{1}{l|}{0.6157/0.7356} &  0.7243 &\multicolumn{1}{l|}{0.3197} & \multicolumn{1}{l|}{0.3903/0.3195} & 0.3358 \\ \cline{2-11} 
                         & 180000       &\multicolumn{1}{l|}{21.6080} & \multicolumn{1}{l|}{18.3553/21.6080} & 21.0473 & \multicolumn{1}{l|}{0.7621} & \multicolumn{1}{l|}{0.6584/0.7621} &  0.7340  &\multicolumn{1}{l|}{0.2938} & \multicolumn{1}{l|}{0.3527/0.2938} &  0.3221 \\ \hline
\multirow{4}{*}{Truck} & 45000        &\multicolumn{1}{l|}{21.1060} & \multicolumn{1}{l|}{13.8701} & 21.1060  &  \multicolumn{1}{l|}{0.7070} & \multicolumn{1}{l|}{0.5597} &    0.7070 &\multicolumn{1}{l|}{0.3802} & \multicolumn{1}{l|}{0.4605} &  0.3802   \\ \cline{2-11} 
                         & 90000        &\multicolumn{1}{l|}{22.5276} & \multicolumn{1}{l|}{14.8729} & 22.5652  & \multicolumn{1}{l|}{0.7673} & \multicolumn{1}{l|}{0.5751} &  0.77126 &\multicolumn{1}{l|}{0.3151} & \multicolumn{1}{l|}{0.4352} & 0.3108 \\ \cline{2-11} 
                         & 135000       &\multicolumn{1}{l|}{23.2394} & \multicolumn{1}{l|}{16.1043} & 22.902 & \multicolumn{1}{l|}{0.7994} & \multicolumn{1}{l|}{0.6259} & 0.7909  &\multicolumn{1}{l|}{0.2753} & \multicolumn{1}{l|}{0.3846} & 0.2840 \\ \cline{2-11} 
                         & 180000       &\multicolumn{1}{l|}{23.6760} & \multicolumn{1}{l|}{17.1049} & 23.0717 & \multicolumn{1}{l|}{0.8193} & \multicolumn{1}{l|}{0.6640} &  0.8006  &\multicolumn{1}{l|}{0.2481} & \multicolumn{1}{l|}{0.3469} &  0.2682 \\ \hline
\end{tabular}
}
\end{table}
% In~\autoref{fig:trained-splats}, we show the trained scene with different densification thresholds, pruning frequency, and other parameter to limit the total number of splats. 
\begin{table}[]
\caption{With segmentation.}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|lll|lll|lll|}
\hline
\multirow{2}{*}{}        & \multirow{2}{*}{\# of splats} & \multicolumn{3}{l|}{psnr} & \multicolumn{3}{l|}{ssim} & \multicolumn{3}{l|}{lpips} \\ \cline{3-11} 
                  &                               & \multicolumn{1}{l|}{separate} & \multicolumn{1}{l|}{sort} & layered & \multicolumn{1}{l|}{separate} & \multicolumn{1}{l|}{sort} & layered      & \multicolumn{1}{l|}{separate} & \multicolumn{1}{l|}{sort} & layered       \\ \hline
\multirow{4}{*}{figurines} & 45000        &\multicolumn{1}{l|}{21.228} & \multicolumn{1}{l|}{} &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &    &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &     \\ \cline{2-11} 
                         & 90000        &\multicolumn{1}{l|}{22.281} & \multicolumn{1}{l|}{} &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \cline{2-11} 
                         & 135000       &\multicolumn{1}{l|}{23.938} & \multicolumn{1}{l|}{} &   &  \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &   &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \cline{2-11} 
                         & 180000       &\multicolumn{1}{l|}{24.657} & \multicolumn{1}{l|}{} & & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &    &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &   \\ \hline
\multirow{4}{*}{ramen} & 45000        &\multicolumn{1}{l|}{25.236} & \multicolumn{1}{l|}{} &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &    &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &     \\ \cline{2-11} 
                         & 90000        &\multicolumn{1}{l|}{27.099} & \multicolumn{1}{l|}{} &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \cline{2-11} 
                         & 135000       &\multicolumn{1}{l|}{27.499} & \multicolumn{1}{l|}{} &   &  \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &   &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \cline{2-11} 
                         & 180000       &\multicolumn{1}{l|}{27.787} & \multicolumn{1}{l|}{} & & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &    &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &   \\ \hline
\multirow{4}{*}{teatime} & 45000        &\multicolumn{1}{l|}{27.588} & \multicolumn{1}{l|}{} &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &     &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &     \\ \cline{2-11} 
                         & 90000        &\multicolumn{1}{l|}{28.016} & \multicolumn{1}{l|}{} &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &   &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \cline{2-11} 
                         & 135000       &\multicolumn{1}{l|}{28.476} & \multicolumn{1}{l|}{} &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &   &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \cline{2-11} 
                         & 180000       &\multicolumn{1}{l|}{28.912} & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &    &\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &   \\ \hline


\end{tabular}
}
\end{table}
\begin{figure}[htbp]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[scale=0.25]{seg.pdf}
  \caption{With segmentation}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
\includegraphics[scale=0.25]{no_seg.pdf}
  \caption{Without segmentation}
\end{subfigure}
\caption{Visual quality (SSIM) with splats}%\vspace{-15pt}
\label{fig:diff}
% \end{wrapfigure}
\end{figure}

\begin{figure}
    \begin{subfigure}[b]{0.6\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/ssim_line.png}
        % \caption{}
        \label{}
    \end{subfigure}
    % ~~~
    \begin{subfigure}[b]{0.25\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/variables_legend.png}
        % \caption{}
        \label{}
    \end{subfigure}
    \caption{Visual quality (SSIM) with splats sorted by different combinations of variables and rendered with different accumulated percentages.}
    \label{fig:sorted-splats}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/ssim_combine_line_.png}
    \caption{Visual quality (SSIM) of with different numbers of splats controlled by different combinations of hyperparameters.}
    \label{fig:trained-splats}
\end{figure}

% \begin{figure}
%     \begin{subfigure}[b]{0.3\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/ref_figures/GT.jpg}
%         \caption{Ground truth}
%         \label{}
%     \end{subfigure}
%     ~~~
%     \begin{subfigure}[b]{0.3\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/ref_figures/LF.jpg}
%         \caption{Low freq.}
%         \label{}
%     \end{subfigure}
%     ~~~
%     \begin{subfigure}[b]{0.3\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/ref_figures/6k.png}
%         \caption{trained 6k}
%         \label{}
%     \end{subfigure}
    
%     \caption{Low frequency image created from ground truth image, and 6k splats trained from the base model. The trained 6k splats has slightly lower SSIM (0.54) compared with the low frequency image (0.56).}
%     \label{fig:ref-view}
% \end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/strategies.png}
    \caption{Three strategies of training with layered scene. Ours-LF trains the first-layered scene with low-frequency images and freezes the first layer and continues to train the second-layered scene. Ours-GT performs a similar strategy to Ours-LF except for using ground truth images when creating the first layer. Ours combined creates two layers of the scene with two separate training processes, one with low-frequency images and another with complemented high-frequency images.}
    \label{fig:trained-strategies}
\end{figure}

Inspired by the trained results that yield higher visual quality, we seek to create layered 3D scenes progressively during the training process. Three strategies are studied as we show in ~\autoref{fig:trained-strategies}.
